The Square Root Agreement Rule for Incentivizing Truthful Feedback on Online Platforms

A major challenge in obtaining evaluations of products or services on e-commerce platforms is eliciting informative responses in the absence of verifiability. This paper proposes the Square Root Agreement Rule (SRA): a simple reward mechanism that incentivizes truthful responses to objective evaluations on such platforms. In this mechanism, an agent gets a reward for an evaluation only if her answer matches that of her peer, where this reward is inversely proportional to a popularity index of the answer. This index is defined to be the square root of the empirical frequency at which any two agents performing the same evaluation agree on the particular answer across evaluations of similar entities operating on the platform. Rarely agreed-upon answers thus earn a higher reward than answers for which agreements are relatively more common. We show that in the many tasks regime, the truthful equilibrium under SRA is strictly payoff-dominant across large classes of natural equilibria that could arise in these settings, thus increasing the likelihood of its adoption. While there exist other mechanisms achieving such guarantees, they either impose additional assumptions on the response distribution that are not generally satisfied for objective evaluations or they incentivize truthful behavior only if each agent performs a prohibitively large number of evaluations and commits to using the same strategy for each evaluation. SRA is the first known incentive mechanism satisfying such guarantees without imposing any such requirements. Moreover, our empirical findings demonstrate the robustness of the incentive properties of SRA in the presence of mild subjectivity or observational biases in the responses. These properties make SRA uniquely attractive for administering reward-based incentive schemes (e.g., rebates, discounts, reputation scores, etc.) on online platforms.

==> commands.tex <==
\newcommand{\newrj}[1]{{\color{blue} #1}}
\newcommand{\delrj}[1]{{\color{blue} \sout{#1}}}
\newcommand{\mexp}{{m_{\tiny {\rm xplr}}}}
\newcommand{\newvj}[1]{{\color{red} #1}}
\newcommand{\delvj}[1]{{\color{red} \sout{#1}}}

\newcommand{\newyk}[1]{{\color{green} #1}}
\newcommand{\delyk}[1]{{\color{green} \sout{#1}}}

\newcommand{\cW}{\mathcal{W}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cXi}{\Xi}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\bcS}{\overline{\mathcal{S}}}
\newcommand{\bcB}{\overline{\mathcal{B}}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\bcD}{\overline{\mathcal{D}}}
\newcommand{\bcM}{\overline{\mathcal{M}}}
\newcommand{\bcXi}{\overline{\Xi}}
\newcommand{\tcXi}{\tilde{\cX}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cPdiff}{{\mathcal{P}_{\tiny {\rm diff}}}}
\newcommand{\cCd}{{\mathcal{C}_{\textup{d}}}}
\newcommand{\cCe}{{\mathcal{C}_{\textup{e}}}}
\newcommand{\Weak}{\textup{Weak}}
\newcommand{\Str}{\textup{Str}}
\newcommand{\MLE}{\textup{MLE}}
\newcommand{\MAP}{\textup{MAP}}
\newcommand{\ecl}{ $}
\newcommand{\ecr}{$ }
\newcommand{\DEEMplus}{\ensuremath{\textrm{DEEM}^+}\,}
\newcommand{\tDEEM}{{{\textup{\tiny DEEM}_N}}}

\newcommand{\eps}{\varepsilon}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\union}{\ensuremath{\bigcup}}
\newcommand{\eq}{{\rm eq}}
\newcommand{\comps}{\ensuremath{\mathbb{C}}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\ints}{\ensuremath{\mathbb{Z}}}
\newcommand{\diag}{\ensuremath{\operatorname{diag}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\renewcommand{\P}{\ensuremath{\mathbb{P}}}

\newcommand{\disp}[1]{\ensuremath{\displaystyle{#1}}}
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\v}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}
\renewcommand{\b}[1]{\ensuremath{\overline{#1}}}
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\renewcommand{\Re}{\ensuremath{\operatorname{Re}}}
\renewcommand{\mod}{\ensuremath{\operatorname{mod}}}
\newcommand{\cJ}{\ensuremath{\mathcal{J}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cS}{\ensuremath{\mathcal{J}}}
\newcommand{\Sk}{\ensuremath{\mathcal{S}}}
\newcommand{\cC}{\ensuremath{\mathcal{I}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\bV}{\ensuremath{\overline{V}}}
\newcommand{\ls}{\textup{limsup}}
\newcommand{\com}{{\textup{c}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}


\renewcommand{\c}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\av}{\rm{\tiny av}}
\newcommand{\uX}{{\underline{X}}}
\newcommand{\ux}{{\underline{x}}}
\newcommand{\var}[1]{\textup{Var}(#1)}
\newcommand{\Ev}{{\cE}}
\newcommand{\ind}{{\mathbb{I}}}
\newcommand{\Po}{\textup{Poisson}}
\newcommand{\Bern}{\textup{Bernoulli}}
\newcommand{\Binom}{\textup{Binomial}}
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\rmb}{{\eta}}
\newcommand{\tg}{{\tilde{\gamma}}}
\newcommand{\tilh}{{\tilde{h}}}
\newcommand{\TV}{{\textup{\tiny TV}}}
\newcommand{\appl}{{\mathcal{S}}}
\newcommand{\pr}{{\textup{Pr}}}
\newcommand{\KL}{{\textup{KL}}}
\definecolor{darkjunglegreen}{rgb}{0.1, 0.14, 0.13}
\newcommand{\yk}[1]{{\color{ForestGreen} [YK: #1]}}
\newcommand{\ykadd}[1]{{\color{ForestGreen} #1}}
\newcommand{\vjmod}[1]{{\color{Magenta} #1}}
\newcommand{\rj}[1]{{\color{blue} [RJ: #1]}}
\newcommand{\vj}[1]{{\color{Magenta} [VJ: #1]}}
\newcommand{\approxt}[1]{\ensuremath{\stackrel{#1}{\approx}}}
\newcommand{\piwho}{{\underline{\pi}}}
\newcommand{\unu}{{\underline{\nu}}}
\newcommand{\echide}[1]{}
\newcommand{\cJfull}{{\cJ^*_{\tiny {\rm full}}}}
\newcommand{\ty}{{\tilde{y}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\edit}[1]{{\color{blue}#1}}
\newcommand{\ub}{{\underline{b}}}
\newcommand{\ob}{{\overline{b}}}

==> experiment.tex <==
\section{Experiments}\label{sec:experiment}
Motivated by the significant emphasis on simplicity of mechanisms in the community~\cite{rubinsteincomplexity, li2015obviously, simonsworkshop}, we performed experiments on the Amazon Mechanical Turk crowdsourcing platform to test the `understandability' or `simplicity' of the structure of our mechanisms as compared to prior art. By simplicity, we roughly mean the ability of the mechanism to induce optimal behavior in agents who are presented with it.  Indeed, ``simplicity'' of the mechanism bears intrinsic value and several applications demand
an understanding of the underlying mechanism: for instance, students wish to know how their
grades are computed, voters wish to know what electoral system is used etc. In what follows, we first describe the experimental setup. Alongside, we also detail the various challenges associated to such a study on Amazon Mechanical Turk and our approaches in overcoming these challenges, which may be of independent interest. Subsequently, we detail the outcomes of the experiment.

\subsection{Experimental setup and challenges}

There are several challenges in designing experiments to study such a characteristic of these mechanisms. Tasks on MTurk are usually objectively verifiable and include image recognition, transcription and matching tasks ~\cite{raykar2010learning}. As a consequence, workers may expect that their work will be verified and rewarded according to their objective accuracy~\cite{shah2015double}. This feature introduces a significant bias for testing incentive compatible mechanisms, as workers have a tendency to report the truth~\cite{gao2014trick}. This effect is amplified when the worker himself or herself is the ``agent'' in the mechanism. Moreover, in order to garner interest from worker, and thereby obtain quality data for the experiment, it is quite essential to make the task interesting~\cite{kaufmann2011more, buhrmester2011amazon}.

In order to address these issues, we present the worker with a game-like setting, where he or she interacts with the experiment via a character (see Figure~\ref{fig:platform} for an example). The goal of the worker is to maximize the payment obtained by the character. We explicitly account for the worker's bias  through the introduction of an `inverted mechanism' for each of our candidate mechanisms, that results from a trivial modification in which all the payments to the agent in the original mechanism are presented as penalties to the worker (over a base reward that ensures that the net payments are non-negative). Hence in these inverted mechanisms, truth-telling is no longer an optimal strategy: in the binary setting, lying is an optimal strategy. Any worker is shown either the normal or the inverted setting, chosen uniformly at random. We also perform an additional randomization of the signal (``A'' or ``B'') observed by the character in the experiment. The game-based setting is further made interesting via illustrations, examples, and simple-to-understand language for the mechanism descriptions. 


We compared the HET-OA mechanism of the present paper with the mechanism of~\cite{radanovic2015incentives} (which we will denote as RF15).\footnote{The mechanism descriptions, data and a link to the actual survey are available at\\ \url{https://eecs.berkeley.edu/~nihar/data/nogold}}

In more detail, the experiment was structured as follows:
\begin{itemize}
\item
Upon visiting the platform, workers are presented with a fictional character ``Sam", whom they will help. Sam's observation (ground truth) is provided to the worker, as well as a question eliciting that observation.
%
\item In the setting, Sam is the grader for an essay in high school, and the principal of the school has announced a reward/penalty according to the quality of grades given by each student. The goal of the worker is to help Sam choose the grade (out of $\{A,B\}$) that will maximize Sam's reward (or minimize Sam's penalty).
%
\item
Each worker is now presented with one of the eight settings (we sample, uniformly at random, which mechanism to present, whether to invert it and which private signal to show) at random and asked whether Sam should answer the question truthfully in order to maximize his payoff assuming everyone else answers truthfully. Each worker only interacts with one setting to minimize possible bias.
%
\item
In addition to providing a (binary) recommendation for Sam, workers are also asked to provide a brief justification.
\end{itemize}
Note that the worker is explained the mechanism but is not told whether the mechanism is attempting to induce the truth or a lie from the worker. Each worker is offered a fixed payment of 30 cents, and contingent on giving the correct answer and a reasonable explanation, an additional bonus of the same amount.


\subsection{Mechanism Descriptions}
Since our goal was to gauge the `understandability` of our mechanisms in the general population, we did not wish to restrict our experiment to agents with a background in mathematics or quantitative sciences. This consequently meant that we had to explain both mechanisms without any mathematical expressions, beyond simple operations like addition and multiplication. %We first described the general idea in informal language, guiding our agents through the reasoning process.  
We presented our mechanism by means of a lookup table and presented the RF mechanism (where there is no intuitive use for such a table) with a sequence of 3 steps of simple addition. %It is interesting to note that our mechanism relied on division, which is a more computationally intensive task than addition used in RF. 
Both mechanisms were accompanied with an example scenario where the payment computation steps are shown along with the final payment.

In the appendix, we present the exact text of the description of the mechanisms given to the workers along with the belief structure of the fictional character. This allowed us to quickly categorize their answers as correct or incorrect for our analysis.

\subsection{Results and analysis}
\begin{figure}
\centering
\subfigure[Illustration of the interface presented to the workers.]{\includegraphics[width = .37 \textwidth]{fig_platform}
\label{fig:platform}
}\qquad
%
\subfigure[Fraction of workers who answered correctly (that is, according to the requirements of that mechanism).]{
\includegraphics[width = .48\textwidth]{experimental_results}
\label{fig:experimental_results}
}
\caption{The platform and the results from experiments on Amazon Mechanical Turk comparing the RF mechanism~\cite{radanovic2015incentives} and the HET-OA mechanism proposed in the present paper. The difference between the two mechanisms is statistically significant ($p < 0.05$).}
\end{figure}

Figure~\ref{fig:experimental_results} plots the results from the experiments, showing the fraction of workers who answered correctly (that is, according to what the mechanism was designed to incentivize). We obtained a total of 223 workers, with 114 workers being shown our mechanism and 109 workers shown the RF mechanism. 

In more detail, the number of workers ($n$) and the fraction of correct responses ($\mu$) and the standard error of the mean ($\epsilon$) associated to each sub-class of the tasks is as follows: 
\begin{center}
\begin{tabular}{|c|ccc|}
\hline
Mechanism & $n$ & $\mu$ & $\epsilon$\\
\hline
HET-OA & 61 & 0.803 & 0.051\\
Inverted HET-OA & 53 & 0.528 & 0.069\\
RF & 60 & 0.500 & 0.065\\
Inverted RF & 49 & 0.592 & 0.070\\
\hline
\end{tabular}
\end{center}

Observe from the table that on average, the workers' responses are more accurate under HET-OA than RF. We employ the standard two-sample t-test~\cite{ttest} between the two sets of data in order to investigate whether this difference is statistically significant or not. The t-test is used to test whether the samples in two sets of data are drawn from an underlying distribution with identical means (the null hypothesis) or not (the alternative hypothesis). In our case, the mean is simply the mean of a Bernoulli distribution that dictates the likelihood of a worker's response being correct. The t-test reveals that HET-OA mechanism elicited a statistically significant number of more correct responses (with a p-value of $ 0.02$) as compared to RF, indicating that the mechanism proposed in this paper was more understandable to the workers as compared to the RF mechanism. 
%In addition, we also elicited comments from the workers regarding their reasoning behind their choices, and the comments also indicate confusion due to the higher complexity of the RF mechanism.\footnote{The full list of comments are available at\\ \url{https://eecs.berkeley.edu/~nihar/data/nogold}}

All in all, these experiments indicate, in a statistically significant manner, that output agreement-type mechanisms with popularity-scaled rewards such as those proposed in the present paper are more intuitive and understandable, and hence more successful in inducing truthful behavior.
